Urban Air Pollution Forecasting: a Machine Learning Approach leveraging Satellite Observations and Meteorological Forecasts

Air pollution poses a significant threat to public health and well-being, particularly in urban areas. This study introduces a series of machine-learning models that integrate data from the Sentinel-5P satellite, meteorological conditions, and topological characteristics to forecast future levels of five major pollutants. The investigation delineates the process of data collection, detailing the combination of diverse data sources utilized in the study. Through experiments conducted in the Milan metropolitan area, the models demonstrate their efficacy in predicting pollutant levels for the forthcoming day, achieving a percentage error of around 30%. The proposed models are advantageous as they are independent of monitoring stations, facilitating their use in areas without existing infrastructure. Additionally, we have released the collected dataset to the public, aiming to stimulate further research in this field. This research contributes to advancing our understanding of urban air quality dynamics and emphasizes the importance of amalgamating satellite, meteorological, and topographical data to develop robust pollution forecasting models.

==> sections/3-methodology_trf.tex <==
The methodology proposed in this work adopts a transformer-based neural architecture comprising an encoder-decoder approach. The transformer architecture was originally proposed for natural language processing tasks, but its attention-based structure makes it well-suited for sequence data analysis across various domains. In the proposed architecture, the encoder processes the series of last available measurements, while the decoder handles meteorological forecast data, combining it with the encoder's output to generate predictions for each subsequent day. An overview of the model architecture is reported in Figure \ref{fig:schema}.

The transformer model receives four distinct inputs: dynamic, static, temporal and forecast data. Dynamic data comprises sources that vary daily, such as satellite and meteorological data, presented as a time series of $T_p$ days each with $F_d$ features. Static data encompasses $F_s$ topological information of the area where dynamic data is measured and as mentioned in previous sections is constant throughout the whole time series. Forecast data provides information about the weather conditions expected in the days to come and is received as a time series of $T_f$ timesteps each with $F_f$ features. Temporal data provides instead insights into the reference period of the $T_p + T_F$ days contained within the dynamic and forecast data. This is achieved through sinusoidal encoding of the day of the year, month of the year, and day of the week, aiding the model in identifying recurring patterns based on annual seasonality or weekly patterns. To harmonize the different dimensions of all inputs and to let the model work in a higher dimensional space, all inputs except for static data are first projected into an embedding space of dimension $E$ using separate linear layers. Static data is instead projected to an embedding space of dimension $E_s$. The resulting data is then processed in the following way. The first $T_p$ tokens of temporal data are added to dynamic data, as they are used as the equivalent of positional encoding in the original transformer paper, to add contextual temporal information to dynamic data. The resulting time series is then processed by the encoder which produces an output series that has the same dimension $T_d x E$ as the input one and represents the current state of the area surrounding the station. 

At this point, the last $T_f$ tokens of temporal data are added to projected forecast data to add contextual temporal information also to this source. The resulting series is then processed in the model decoder alongside the encoder output. The encoder-decoder cross-attention mechanism conditions the output for each token in this forecast series on the value of the encoder output summarizing the current condition. As for the encoder, the decoder's output series has the same dimension $T_f x E$ as the input and each token contains information about future days that is the result of the combination of the weather forecast expected for that day and the current status. As the last step, processed static data are repeatedly concatenated into output series to take into account also topological information in the final output. The final series of tokens with dimension  $T_f x 2E$ is processed by a regression head composed of linear layers that estimate the pollutant concentration for each future day. This output is compared to ground station measurements and the model is updated using the Mean Squared Error (MSE) loss function, expressed as $(p - \hat{p})^2$ where $p$ and $\hat{p}$ are respectively model output and ground truth measurements.
